MoVE-KD: Knowledge Distillation for VLMs with Mixture of Visual Encoders

Visual encoders are fundamental components in vision-language models (VLMs), each showcasing unique strengths derived from various pre-trained visual foundation models. To leverage the various capabilities of these encoders, recent studies incorporate multiple encoders within a single VLM, leading to a considerable increase in computational cost. In this paper, we present Mixture-of-Visual-Encoder Knowledge Distillation (MoVE-KD), a novel framework that distills the unique proficiencies of multiple vision encoders into a single, efficient encoder model. Specifically, to mitigate conflicts and retain the unique characteristics of each teacher encoder, we employ low-rank adaptation (LoRA) and mixture-of-experts (MoEs) to selectively activate specialized knowledge based on input features, enhancing both adaptability and efficiency. To regularize the KD process and enhance performance, we propose an attention-based distillation strategy that adaptively weighs the different encoders and emphasizes valuable visual tokens, reducing the burden of replicating comprehensive but distinct features from multiple teachers. Comprehensive experiments on popular VLMs, such as LLaVA and LLaVA-NeXT, validate the effectiveness of our method. Our code is available at: https://github.com/hey-cjj/MoVE-KD.

==> tab/MoVE_v1.1.tex <==
\renewcommand{\multirowsetup}{\centering}
\definecolor{mygray}{gray}{.92}
\definecolor{ForestGreen}{RGB}{34,139,34}
\definecolor{Forestred}{RGB}{220,50,50}
\definecolor{goldenrod}{RGB}{250, 250, 235}
\newcolumntype{a}{>{\columncolor{goldenrod}}c}
\begin{table*}[!h]
    \centering
    % \hspace{2mm}
    \setlength{\tabcolsep}{2.8pt}
    \renewcommand{\arraystretch}{1.6}
    \footnotesize
	\centering
	
    \begin{tabular}{p{2.5cm} c | p{1cm}<{\centering} p{1cm}<{\centering} p{1cm}<{\centering} p{1cm}<{\centering} p{1cm}<{\centering} p{1cm}<{\centering} p{1cm}<{\centering} p{1cm}<{\centering}}
        \shline
        \textbf{Method} & \textbf{LLM} &\textbf{VQA}$^{\text{V2}}$ & \textbf{GQA} &  \textbf{VQA}$^{\text{Text}}$ & \textbf{VizWiz} & \textbf{POPE} & \textbf{SQA}& \textbf{MME} & \textbf{MMB} \\
        \hline
        \rowcolor{mygray}
        \multicolumn{10}{c}{\textit{1.7B Models}} \\
        LLaVA-1.5 \cite{liu2023improvedllava} & MobileLLaMA-1.4B \cite{chu2023mobilevlm}  & 71.5 & 55.4 & 42.6 & 28.6 & 84.3 & 56.0 & 1145.7 & 47.0 \\
        + MoVE-KD-v1.0  & MobileLLaMA-1.4B \cite{chu2023mobilevlm}  & \underline{72.9} & \underline{56.6} & \underline{43.4} & \textbf{32.1} & \underline{84.8} & \underline{56.1} & \underline{1182.3} & \underline{47.4}\\
        + MoVE-KD-v1.1  & MobileLLaMA-1.4B 
        \cite{chu2023mobilevlm}  & \textbf{73.8} & \textbf{57.7} & \textbf{44.3} & \underline{29.3} & \textbf{86.1} & \textbf{57.3} & \textbf{1188.4} & \textbf{48.8}\\
        \hline
        
        \rowcolor{mygray}
        \multicolumn{10}{c}{\textit{7B Models}} \\
        LLaVA-1.5 \cite{liu2023improvedllava} & Vicuna-7B \cite{zheng2023judging} & 78.5 & 62.0 & 58.2 & 50.0 & 85.9 & 66.8 & 1510.7 & 64.3 \\
        + MoVE-KD-v1.0  & Vicuna-7B \cite{zheng2023judging} & \underline{79.5} & \underline{63.2} & \underline{58.3} & \underline{52.3} & \textbf{86.9} & \underline{69.3} & \textbf{1524.5} & \underline{66.3} \\
        + MoVE-KD-v1.1  & Vicuna-7B \cite{zheng2023judging} & \textbf{79.9} & \textbf{63.9} & \textbf{59.6} & \textbf{52.7} & \underline{86.3} & \textbf{69.8} & 1509.1 & \textbf{67.4} \\
        \hline

        \rowcolor{mygray}
        \multicolumn{10}{c}{\textit{13B Models}} \\
        LLaVA-1.5 \cite{liu2023improvedllava} & Vicuna-13B \cite{zheng2023judging} & 80.0 & 63.3 & 61.3 & 53.6 & 85.9 & 71.6 & 1531.3 & 67.7 \\
        + MoVE-KD-v1.0 & Vicuna-13B \cite{zheng2023judging} & \underline{80.6} & \textbf{64.2} & 59.7 & \underline{55.7} & 85.7 & \textbf{73.2} & \underline{1568.1} & \textbf{70.2} \\
        + MoVE-KD-v1.1 & Vicuna-13B \cite{zheng2023judging} & \textbf{80.8} &  \underline{63.9} & \underline{61.1} & \textbf{57.5} & \textbf{86.3} & \underline{71.8} & \textbf{1568.3} & \underline{69.7} \\
        \hline
       
        \shline
	\end{tabular}
     \vspace{-2mm}
     \caption{\textbf{Performance of MoVE-KD-v1.0 and MoVE-KD-v1.1}}
    \vspace{-2mm}
	\label{tab:move_1.1}
\end{table*}

==> tab/X_mse.tex <==
\renewcommand{\multirowsetup}{\centering}
\definecolor{mygray}{gray}{.92}
\definecolor{ForestGreen}{RGB}{34,139,34}
\definecolor{Forestred}{RGB}{220,50,50}
\definecolor{goldenrod}{RGB}{250, 250, 235}
\newcolumntype{a}{>{\columncolor{goldenrod}}c}
\begin{table*}[!h]
    \centering
    % \hspace{2mm}
    \setlength{\tabcolsep}{2.8pt}
    \renewcommand{\arraystretch}{1.6}
    \footnotesize
	\centering
	
    \begin{tabular}{p{3cm} c | p{1cm}<{\centering} p{1cm}<{\centering} p{1cm}<{\centering} p{1cm}<{\centering} p{1cm}<{\centering} p{1cm}<{\centering} p{1cm}<{\centering} p{1cm}<{\centering}}
        \shline
        \textbf{Method} & \textbf{LLM} &\textbf{VQA}$^{\text{V2}}$ & \textbf{GQA} &  \textbf{VQA}$^{\text{Text}}$ & \textbf{VizWiz} & \textbf{POPE} & \textbf{SQA}& \textbf{MME} & \textbf{MMB} \\
        \hline
        \rowcolor{mygray}
        \multicolumn{10}{c}{\textit{1.7B Models}} \\
        LLaVA-1.5 \cite{liu2023improvedllava} & MobileLLaMA-1.4B \cite{chu2023mobilevlm}  & 71.5 & 55.4 & 42.6 & 28.6 & 84.3 & 56.0 & 1145.7 & 47.0 \\
        + MSE & MobileLLaMA-1.4B \cite{chu2023mobilevlm}  & 72.0 & 55.8 & 42.5 & 29.3 & 84.2 & 55.4 & 1161.8 & 47.1 \\
        \rowcolor{goldenrod}
        + MoVE-KD \texttt{\scriptsize{(Ours)}} & MobileLLaMA-1.4B \cite{chu2023mobilevlm}  & \textbf{72.9} & \textbf{56.6} & \textbf{43.4} & \textbf{32.1} & \textbf{84.8} & \textbf{56.1} & \textbf{1182.3} & \textbf{47.4}\\
        \hline
        
        \rowcolor{mygray}
        \multicolumn{10}{c}{\textit{7B Models}} \\
        InstructBLIP \cite{liu2024visual} & Vicuna-7B \cite{zheng2023judging} & - & 49.2 & 50.1 & 34.5 & - & 60.5 & - & 36 \\
        Qwen-VL \cite{bai2023qwen} & Qwen-7B \cite{bai2023qwen} & 78.8 & 59.3 & 63.8 & 35.2 & - & 67.1 & 1487.5 & 38.2\\
        \hline
        LLaVA-1.5 \cite{liu2023improvedllava} & Vicuna-7B \cite{zheng2023judging} & 78.5 & 62.0 & 58.2 & 50.0 & 85.9 & 66.8 & 1510.7 & 64.3 \\
        + MSE & Vicuna-7B \cite{zheng2023judging} & 79.0 & 62.4 & 56.7 & 50.9 & 84.7 & 67.6 & 1507.6 & 62.9 \\
        + RADIO \cite{ranzinger2024radio} & Vicuna-7B \cite{zheng2023judging} & 76.3 & 63.0 & 56.3 & - & 86.2 & - & - & - \\
        \rowcolor{goldenrod}
        + MoVE-KD \texttt{\scriptsize{(Ours)}} & Vicuna-7B \cite{zheng2023judging} & \textbf{79.5} & \textbf{63.2} & \textbf{58.3} & \textbf{52.3} & \textbf{86.9} & \textbf{69.3} & \textbf{1524.5} & \textbf{66.3} \\
        \hline
        LLaVA-NeXT \cite{liu2024llavanext} & Vicuna-7B \cite{zheng2023judging} & 81.8 & 64.2 & 64.9 & 57.6 & 86.5 & 70.1 & 1519.0 & 67.4 \\
        + MSE & Vicuna-7B \cite{zheng2023judging} & 82.0 & 63.5 & 63.1 & 57.2 & 86.4 & 70.3 & 1526.9 & 67.0 \\
        \rowcolor{goldenrod}
        + MoVE-KD \texttt{\scriptsize{(Ours)}} & Vicuna-7B \cite{zheng2023judging} & \textbf{82.3} & \textbf{64.5} & 63.7 & \textbf{58.0} & \textbf{86.7} & \textbf{70.7} & \textbf{1537.2} & \textbf{67.6} \\
        \hline

        \rowcolor{mygray}
        \multicolumn{10}{c}{\textit{13B Models}} \\
        InstructBLIP \cite{liu2024visual} & Vicuna-13B \cite{zheng2023judging} & - & 49.5 & 50.7 & 33.4 & 78.9 & 63.1 & 1212.8 & - \\
        \hline
        LLaVA-1.5 \cite{liu2023improvedllava} & Vicuna-13B \cite{zheng2023judging} & 80.0 & 63.3 & 61.3 & 53.6 & 85.9 & 71.6 & 1531.3 & 67.7 \\
        \rowcolor{goldenrod}
        + MSE & Vicuna-13B \cite{zheng2023judging} & 80.1 & 63.7 & 58.4 & 54.6 & 84.7 & 71.9 & 1543.3 & 68.8 \\
        + MoVE-KD \texttt{\scriptsize{(Ours)}} & Vicuna-13B \cite{zheng2023judging} & \textbf{80.6} & \textbf{64.2} & 59.7 & \textbf{55.7} & 85.7 & \textbf{73.2} & \textbf{1568.1} & \textbf{70.2} \\
        \hline
        LLaVA-NeXT \cite{liu2024llavanext} & Vicuna-13B \cite{zheng2023judging} & 82.8 & 65.4 & 67.1 & 60.5 & 86.2 & 73.6 & 1575.0 & 70 \\
        + MSE & Vicuna-13B \cite{zheng2023judging} & 82.4 & 65.1 & 64.5 & 60.7 & 86.3 & 73.4 & 1568.4 & 70.3 \\
        \rowcolor{goldenrod}
        + MoVE-KD \texttt{\scriptsize{(Ours)}} & Vicuna-13B \cite{zheng2023judging} & \textbf{83.1} & \textbf{65.7} & 65.8 & \textbf{60.9} & \textbf{86.8}  & \textbf{73.7} & \textbf{1579.3} & \textbf{70.6}  \\

        \shline
	\end{tabular}
     \vspace{-2mm}
     \caption{\textbf{Performance of MoVE-KD and other methods} (inlcude MSE KD.) }
    \vspace{-2mm}
	\label{tab:X_mse}
\end{table*}

==> tab/rebuttal_abla.tex <==
\begin{table}[!h]
    \centering
    \setlength{\tabcolsep}{1.8pt} % 缩小列间距以适应半栏
    \renewcommand{\arraystretch}{1.4} % 缩小行距
    \scriptsize  % 使用更小的字体
	
    \vspace{-3mm}
    
    \begin{tabular}{p{1.3cm}<{\centering} | p{0.7cm}<{\centering} p{0.7cm}<{\centering} p{0.9cm}<{\centering} p{0.8cm}<{\centering} p{0.7cm}<{\centering} p{0.6cm}<{\centering} p{0.7cm}<{\centering} p{0.7cm}<{\centering} }
        \shline
         \textbf{Methods} &\textbf{VQA}$^{\text{V2}}$ & \textbf{GQA} &  \textbf{VQA}$^{\text{Text}}$ & \textbf{VizWiz} & \textbf{POPE} & \textbf{SQA} & \textbf{MME} & \textbf{MMB}\\
        \hline
        Ours   & 79.5 & 63.2 & 58.3 & \textbf{52.3} & 86.9 & \textbf{69.3}  & \textbf{1524.5} & \textbf{66.3} \\
        None-MoLE & 79.1 & 63.4 & 57.1 & 51.8 & 86.3 & 68.7  & 1518.7 & 65.7  \\
       FFN-MoE & 79.7 & 63.6 & 58.8 & 52.0 & 87.4 & 69.2  & 1522.6 & 66.0  \\
       R-2:Q3(1) & 79.3 & 63.1 & 57.8 & 51.6 & 86.6 & 69.0  & 1521.9 & 66.2  \\
       Eagle* & \textbf{80.2} & \textbf{63.9} & \textbf{66.9} & {51.9} & \textbf{88.5} & 68.4  & 1439 & 65.5  \\
        \hline
        \shline
	\end{tabular}
    \vspace{-3mm}
    \caption{Eagle* means Eagle uses the same setup as MoVE-KD.} 
    \label{tab:re_abla}
\end{table}


==> tab/rebuttal_effiiciency.tex <==
% \begin{table}[!h]
%     \centering
%     \setlength{\tabcolsep}{1.8pt} % 缩小列间距以适应半栏
%     \renewcommand{\arraystretch}{1.4} % 缩小行距
%     \scriptsize  % 使用更小的字体
% 	% CLIP: 0.04109 T, EVA: 0.20352 T, ConvNeXt: 0.0045 T
%     % CLIP: 0.04109 T, DINOv2: 0.507 T, SAM: 0.0465 T
% 	% CLIP: 0.04109 T, EVA: 0.20352 T, ConvNeXt: 0.0045 T
    
%     \vspace{-3mm}
    
%     \begin{tabular}{p{1.8cm}<{\centering} | p{1.8cm}<{\centering} p{1.6cm}<{\centering} p{2.5cm}<{\centering} }
%         \shline
%          \textbf{Methods} &\textbf{Params(M)} & \textbf{FLOPs(T)} &  \textbf{Throughput(it/s)}\\
%         \hline
%         Ours   & 327 & 0.25 & 7.7  \\
%         AM-RADIO & 653 & 0.46 & 6.4  \\
%         Eagle* & 1453 & 0.59 & 3.6 \\
%         \hline
%         \shline
% 	\end{tabular}
%     \vspace{-3mm}
%     \caption{Params and FLOPs of the vision encoder for each method, and average throughput on GQA.} 
%     \label{tab:re_effi}
% \end{table}

\begin{wraptable}{r}{0.55\linewidth}  % 调整表格宽度
    \centering
    \setlength{\tabcolsep}{2pt} % 缩小列间距
    \renewcommand{\arraystretch}{1.4} % 缩小行距
    \tiny  % 使用最小的字体
    \vspace{-4mm}  % 调整表格上下间距
    \begin{tabular}{p{0.9cm}<{\centering} | p{0.9cm}<{\centering} p{0.8cm}<{\centering} p{1.2cm}<{\centering} }
        \shline
         Methods & Params(M)$\downarrow$ & FLOPs(T)$\downarrow$ & Throughput(it/s)$\uparrow$\\
        \hline
        Ours   & 327 & 0.25 & 7.7  \\
        AM-RADIO & 653 & 0.36 & 6.4  \\
        Eagle* & 1453 & 0.59 & 3.6 \\
        \hline
        \shline
    \end{tabular}
    \vspace{-3mm}
    \caption{Params and FLOPs of the vision encoder for each method, and average throughput on GQA.}% 让标题字体也变小
    
    \label{tab:re_effi}
    \vspace{-4.5mm}
\end{wraptable}




